ASC: Adaptive Scale Feature Map Compression for Deep Neural Network

Deep-learning accelerators are increasingly in demand; however, their performance is constrained by the size of the feature map, leading to high bandwidth requirements and large buffer sizes. We propose an adaptive scale feature map compression technique leveraging the unique properties of the feature map. This technique adopts independent channel indexing given the weak channel correlation and utilizes a cubical-like block shape to benefit from strong local correlations. The method further optimizes compression using a switchable endpoint mode and adaptive scale interpolation to handle unimodal data distributions, both with and without outliers. This results in 4$\times$ and up to 7.69$\times$ compression rates for 16-bit data in constant and variable bitrates, respectively. Our hardware design minimizes area cost by adjusting interpolation scales, which facilitates hardware sharing among interpolation points. Additionally, we introduce a threshold concept for straightforward interpolation, preventing the need for intricate hardware. The TSMC 28nm implementation showcases an equivalent gate count of 6135 for the 8-bit version. Furthermore, the hardware architecture scales effectively, with only a sublinear increase in area cost. Achieving a 32$\times$ throughput increase meets the theoretical bandwidth of DDR5-6400 at just 7.65$\times$ the hardware cost.

==> Makefile <==
TARGET=main
LATEX_BUILD_CMD=xelatex -synctex=1 -shell-escape -interaction=nonstopmode

default: build

build:
	$(LATEX_BUILD_CMD) $(TARGET).tex
	bibtex main.aux || true
	$(LATEX_BUILD_CMD) $(TARGET).tex
	$(LATEX_BUILD_CMD) $(TARGET).tex | grep 'Warning\|pages'
clean:
	rm -rf *.aux *.log *.gz *.bbl *.blg *.lof *.lot *.toc *.out


==> ack/ack.tex <==
\begin{acknowledgement}%

在這兩年的碩士生涯中，我學習到了如何探索並研究專業領域的知識，同時也讓自己在面對問題時的思維更加清晰。實驗室的生活讓我學會了如何與他人合作並運用所學來達成目標。

首先，我要感謝我的指導教授張添烜老師。不論是在研究或是人生的道路上，他給了我許多寶貴的建議與指導，在我遇到困境時也給予了很多幫助，使我得以順利解決問題。這兩年的求學過程中，有了老師的帶領，我才沒有在研究上迷失方向。另外，我還要感謝范倫達教授以及蔡淳仁教授願意擔任口試委員給予指導，讓我發現研究上可以改進的地方，使我獲益匪淺。

同樣地，我要感謝實驗室的夥伴們，讓我在辛勤的研究過程中獲得了許多快樂。感謝啟豪、立維、鈺涵、仲緯、書宏、敦皓、洪毅在我碩士一年級時的教導，謝謝志嘉、子嘉、洛亘、晏誠這兩年來的協助。謝謝凱捷、楚堯、宗任、奕萱、民瀚、揚展、芳淇、昶裕、東軒、柏瑀、慶林的陪伴。大家相處融洽，互相支持，使研究生活更順利、也更安心。除了實驗室成員，我還要感謝交大男子排球隊與所有球友，讓我在研究辛苦之餘能夠運動調劑身心。

最後，感謝我的爸媽、女友給予我毫無保留的支持與鼓勵，讓我得以順利完成學業，也給予我前進的動力。他們的支持對我來說意義重大。

\end{acknowledgement}

==> thesis_new.tex <==
\ProvidesClass{thesis}[2022/02/25 V2.0]
\NeedsTeXFormat{LaTeX2e}


\DeclareOption*{\PassOptionsToClass{\CurrentOption}{book}}

\newif\ifTHESISOPTIONmaster         \THESISOPTIONmastertrue
\newif\ifTHESISOPTIONphd            \THESISOPTIONphdfalse

\DeclareOption{master}{\THESISOPTIONmastertrue\THESISOPTIONphdfalse}
\DeclareOption{phd}{\THESISOPTIONmasterfalse\THESISOPTIONphdtrue}

\newif\ifTHESISOPTIONen             \THESISOPTIONentrue
\newif\ifTHESISOPTIONzh             \THESISOPTIONzhfalse

\DeclareOption{en}{\THESISOPTIONentrue\THESISOPTIONzhfalse}
\DeclareOption{zh}{\THESISOPTIONenfalse\THESISOPTIONzhtrue}

\newif\ifTHESISOPTIONbinding      \THESISOPTIONbindingfalse
\DeclareOption{binding}{\THESISOPTIONbindingtrue}

\newif\ifTHESISOPTIONreview         \THESISOPTIONreviewfalse
\newif\ifTHESISOPTIONdraft          \THESISOPTIONdrafttrue
\newif\ifTHESISOPTIONfinal          \THESISOPTIONfinalfalse

\DeclareOption{review}{\THESISOPTIONreviewtrue
                       \THESISOPTIONdraftfalse
                       \THESISOPTIONfinalfalse
                       \THESISOPTIONbindingfalse}

\DeclareOption{draft}{\THESISOPTIONreviewfalse
                      \THESISOPTIONdrafttrue
                      \THESISOPTIONfinalfalse
                      \THESISOPTIONbindingfalse}

\DeclareOption{final}{\THESISOPTIONreviewfalse
                      \THESISOPTIONdraftfalse
                      \THESISOPTIONfinaltrue
                      \THESISOPTIONbindingtrue}

\newif\ifTHESISOPTIONwatermark      \THESISOPTIONwatermarkfalse
\DeclareOption{watermark}{\THESISOPTIONwatermarktrue}

\ProcessOptions
\LoadClass[a4paper,12pt,oneside]{book}


\usepackage[BoldFont, SlantFont, CJKchecksingle, CJKmath=true]{xeCJK}
\usepackage{fontspec}     %
\usepackage{ifplatform}   %
\usepackage{indentfirst}  %
\usepackage{setspace}     %
\usepackage{tikz}         %
\usepackage{eso-pic}      %
\usepackage[xetex, hidelinks]{hyperref}  %
\usepackage{geometry}     %
\usepackage{emptypage}    %
\usepackage{afterpage}    %
\usepackage{lipsum}       %
\usepackage{verbatim}     %
\usepackage[retainorgcmds]{IEEEtrantools}  %
\usepackage{xCJKnumb}     %
\usepackage{titlesec}     %
\usepackage{titletoc}     %
\usepackage{tocloft}	  %
\usepackage{caption}	  %
\usepackage[labelformat=simple]{subcaption} %
\usepackage[chapter]{algorithm}  %


\ifTHESISOPTIONbinding  %
  \geometry{left=3 cm, right=2 cm, top=3 cm, bottom=3 cm}%
\else
  \geometry{left=2.5 cm, right=2.5 cm, top=3 cm, bottom=3 cm}%
\fi

\pagestyle{plain}
\setlength{\footskip}{1.5cm}

\doublespacing


\newcommand{\mainfont}[1]{%
\ifx&#1&%
  \setmainfont[Ligatures=TeX]{Times New Roman}
\else
  \setmainfont[Ligatures=TeX]{#1}
\fi
}

\newcommand{\sansfont}[1]{%
\ifx&#1&%
  \setsansfont[Ligatures=TeX]{Arial}
\else
  \setsansfont[Ligatures=TeX]{#1}
\fi
}


\newcommand{\mainfontzh}[1]{%
\ifx&#1&%
  \ifwindows  %
    \setCJKmainfont{DFKai-SB}  %
  \else\iflinux  %
    \setCJKmainfont{AR PL UKai TW}  %
  \else\ifmacosx  %
    \setCJKmainfont{Kaiti TC Regular}  %
  \else  %
    \setCJKmainfont{DFKai-SB}
  \fi\fi\fi
\else
  \setCJKmainfont{#1}
\fi
}

\newcommand{\sansfontzh}[1]{%
\ifx&#1&%
  \ifwindows  %
    \setCJKsansfont{PMingLiU}  %
  \else\iflinux  %
    \setCJKsansfont{AR PL UMing TW}  %
  \else\ifmacosx  %
    \setCJKsansfont{LiSong Pro}  %
  \else  %
    \setCJKsansfont{PMingLiU}
  \fi\fi\fi
\else
  \setCJKsansfont{#1}
\fi
}

\XeTeXlinebreaklocale "zh"
\XeTeXlinebreakskip = 0pt plus 1pt


\def\titlezh#1{\gdef\@titlezh{#1}}

\def\degreeyear#1{\gdef\@degreeyear{#1}}
\def\degreemonth#1{\gdef\@degreemonth{#1}}

\def\degreeyearzh#1{\gdef\@degreeyearzh{#1}}

\def\nation#1{\gdef\@nation{#1}}

\def\yearmonth#1{\gdef\@yearmonth{#1}}

\def\degree#1{\gdef\@degree{#1}}

\def\field#1{\gdef\@field{#1}}

\def\thesistype#1{\gdef\@thesistype{#1}}

\def\thesistypezh#1{\gdef\@thesistypezh{#1}}

\def\institute#1{\gdef\@institute{#1}}

\def\institutezh#1{\gdef\@institutezh{#1}}

\def\college#1{\gdef\@college{#1}}

\def\university#1{\gdef\@university{#1}}

\def\universityzh#1{\gdef\@universityzh{#1}}

\def\location#1{\gdef\@location{#1}}

\def\advisor#1{\gdef\@advisor{#1}}

\def\advisorzh#1{\gdef\@advisorzh{#1}}

\def\coadvisorA#1{\gdef\@coadvisorA{#1}}

\def\coadvisorAzh#1{\gdef\@coadvisorAzh{#1}}

\def\coadvisorB#1{\gdef\@coadvisorB{#1}}

\def\coadvisorBzh#1{\gdef\@coadvisorBzh{#1}}

\def\authorzh#1{\gdef\@authorzh{#1}}

\def\watermark#1{\gdef\@watermark{#1}}

\def\acktitle#1{\gdef\@acktitle{#1}}

\def\toctitle#1{\gdef\@toctitle{#1}}

\def\loftitle#1{\gdef\@loftitle{#1}}

\def\lottitle#1{\gdef\@lottitle{#1}}

\def\bibtitle#1{\gdef\@bibtitle{#1}}

\def\cvtitle#1{\gdef\@cvtitle{#1}}

\def\loptitle#1{\gdef\@loptitle{#1}}

\def\reservedfrontpages#1{\gdef\@reservedfrontpages{#1}}


\ifTHESISOPTIONmaster
  \thesistype{Master Thesis}%
  \thesistypezh{碩士論文}%
  \degree{Master}%
  \reservedfrontpages{0}%
\else
  \thesistype{Doctoral Dissertation}%
  \thesistypezh{博士論文}%
  \degree{Doctor of Philosophy}%
  \reservedfrontpages{0}%
\fi

\ifTHESISOPTIONzh
  \acktitle{誌謝}%
  \toctitle{目錄}%
  \loftitle{圖目錄}%
  \lottitle{表目錄}%
  \bibtitle{參考文獻}%
  \cvtitle{自傳}%
  \loptitle{著作目錄}%
\else
  \acktitle{Acknowledgement}%
  \toctitle{Table of Contents}%
  \loftitle{List of Figures}%
  \lottitle{List of Tables}%
  \ifTHESISOPTIONmaster
    \bibtitle{References}%
  \else
    \bibtitle{Bibliography}%
  \fi
  \cvtitle{Curriculum Vitae}%
  \loptitle{List of Publications}%
\fi


\renewcommand{\cfttoctitlefont}{\hspace*{\fill}\Huge\bfseries}
\renewcommand{\cftaftertoctitle}{\hspace*{\fill}}
\renewcommand{\cftlottitlefont}{\hspace*{\fill}\Huge\bfseries}
\renewcommand{\cftafterlottitle}{\hspace*{\fill}}
\renewcommand{\cftloftitlefont}{\hspace*{\fill}\Huge\bfseries}
\renewcommand{\cftafterloftitle}{\hspace*{\fill}}

\ifTHESISOPTIONzh
  \renewcommand{\contentsname}{\makebox[3em][s]{\@toctitle}}%
  \renewcommand{\listfigurename}{\makebox[4em][s]{\@loftitle}}%
  \renewcommand{\listtablename}{\makebox[4em][s]{\@lottitle}}%
  \renewcommand{\tablename}{表}%
  \renewcommand{\figurename}{圖}%
\else
  \renewcommand{\contentsname}{\@toctitle}%
  \renewcommand{\listfigurename}{\@loftitle}%
  \renewcommand{\listtablename}{\@lottitle}%
\fi

\ifTHESISOPTIONzh
  \titlecontents{chapter}[0pt]{}%
  {\bfseries\xCJKnumber{\thecontentslabel}、\hspace{0.5em}}{}%
  {\cftdotfill{\cftdotsep}\contentspage}%
\else
  \titlecontents{chapter}[0pt]{}%
  {\bfseries\makebox[1em][l]{\thecontentslabel}\hspace{0.25em}}{}%
  {\cftdotfill{\cftdotsep}\contentspage}%
\fi

\renewcommand\cftbeforetoctitleskip{-0.5cm}
\renewcommand\cftbeforeloftitleskip{-0.5cm}
\renewcommand\cftbeforelottitleskip{-0.5cm}

\def\maketocs{%
\ifTHESISOPTIONreview\else
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@toctitle}}%
  \tableofcontents
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@loftitle}}%
  \listoffigures
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@lottitle}}%
  \listoftables
\fi
}


\ifTHESISOPTIONzh
  \titleformat{\chapter}[block]%
  {\centering\Huge\bfseries}%
  {\xCJKnumber{\thechapter}、\hspace{0.5em}}%
  {0em}{}%
\else
  \titleformat{\chapter}[display]%
  {\centering\Huge\bfseries}%
  {\chaptertitlename\ \thechapter}%
  {0em}{}%
\fi

\titlespacing*{\chapter}{0em}{-40pt}{*6}


\newcommand\BackgroundPicture{%
\ifTHESISOPTIONwatermark
  \ifTHESISOPTIONdraft
    \setlength{\@tempdimb}{.5\paperwidth}%
    \setlength{\@tempdimc}{.5\paperheight}%
    \setlength{\unitlength}{1pt}%
    \put(\strip@pt\@tempdimb,\strip@pt\@tempdimc){%
    \makebox(0,0){\rotatebox{45}{\textcolor[gray]{0.75}%
      {\fontsize{6cm}{6cm}\selectfont{DRAFT}}}}%
    }%
  \fi
  \ifTHESISOPTIONfinal
    \begin{tikzpicture}%
      \node[minimum width=\paperwidth,minimum height=\paperheight,opacity=0.75]%
        {\includegraphics[width=0.4\textwidth]{\@watermark}};%
    \end{tikzpicture}%
  \fi
\fi
}

\let\oldcleardoublepage\cleardoublepage
\renewcommand{\cleardoublepage}{%
  \newpage
  \ClearShipoutPicture
  \oldcleardoublepage
  \AddToShipoutPicture{\BackgroundPicture}%
}


\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}

\def\changemargin#1#2{\list{}{\rightmargin#2\leftmargin#1}\item[]}
\let\endchangemargin=\endlist 

\DeclareRobustCommand{\xCJKalphatozhnum}[1]{%
  \ifnum\strcmp{#1}{A} = 0 一 \else
  \ifnum\strcmp{#1}{B} = 0 二 \else
  \ifnum\strcmp{#1}{C} = 0 三 \else
  \ifnum\strcmp{#1}{D} = 0 四 \else
  \ifnum\strcmp{#1}{E} = 0 五 \else
  \ifnum\strcmp{#1}{F} = 0 六 \else
  \ifnum\strcmp{#1}{G} = 0 七 \else
  \ifnum\strcmp{#1}{H} = 0 八 \else
  \ifnum\strcmp{#1}{I} = 0 九 \else
  \ifnum\strcmp{#1}{J} = 0 十 \else
  \ifnum\strcmp{#1}{K} = 0 十一 \else
  \ifnum\strcmp{#1}{L} = 0 十二 \else
  \ifnum\strcmp{#1}{M} = 0 十三 \else
  \ifnum\strcmp{#1}{N} = 0 十四 \else
  \ifnum\strcmp{#1}{O} = 0 十五 \else
  \ifnum\strcmp{#1}{P} = 0 十六 \else
  \ifnum\strcmp{#1}{Q} = 0 十七 \else
  \ifnum\strcmp{#1}{R} = 0 十八 \else
  \ifnum\strcmp{#1}{S} = 0 十九 \else
  \ifnum\strcmp{#1}{T} = 0 二十 \else 零%
  \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
}


\newcommand{\addBibToContents}{%
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@bibtitle}}%
}

\renewcommand{\bibname}{\makebox[5.5em][s]{\@bibtitle}}


\renewcommand{\thealgorithm}{\arabic{chapter}.\arabic{algorithm}}


\newcommand{\addAppxToContents}{%
\addtocontents{toc}{\protect\setcounter{tocdepth}{0}}
\ifTHESISOPTIONzh
  \titlecontents{chapter}[0pt]{}%
  {\bfseries 附錄\xCJKalphatozhnum{\thecontentslabel}\quad}%
  {}{\cftdotfill{\cftdotsep}\contentspage}%

  \titleformat{\chapter}[block]%
  {\centering\Huge\bfseries}%
  {附錄\xCJKalphatozhnum{\thechapter}\quad}%
  {0em}{}%
\else
  \titlecontents{chapter}[0pt]{}%
  {\bfseries \appendixname\hspace{0.5em}\thecontentslabel\hspace{0.5em}}%
  {}{\cftdotfill{\cftdotsep}\contentspage}%
\fi
}


\renewcommand\thesubfigure{ (\alph{subfigure})}


\def\coverpage
{
  \thispagestyle{empty}%
  \begin{center}
    \fontsize{18}{27}{\@universityzh}\\
    \fontsize{18}{27}{\@institutezh}\\
    \fontsize{18}{27}{\@thesistypezh}\\
    \ifTHESISOPTIONdraft
      \fontsize{18}{27}{初稿}\\
    \fi
    \vspace{2\baselineskip}
    
    \fontsize{14}{21}{\@institute}\\
    \fontsize{16}{24}{\@university}\\
    \fontsize{16}{24}{\@thesistype}\\
    \vspace{3\baselineskip} %

    \fontsize{18}{27}{\@titlezh}\\
    \vspace{0.75\baselineskip}
    \fontsize{18}{27}{\@title}\\
    \vspace{3\baselineskip} %
  
    \singlespacing
    \fontsize{18}{27}
    \begin{center}
    \begin{tabular}{c}%
      {研究生\ :} {\@authorzh \ (\@author)} \vspace{1em}\\%
      {指導教授\ :}{\@advisorzh \ (\@advisor)} \vspace{1em}\\%
      \ifx \@coadvisorAzh \@empty \else
        {\@coadvisorAzh(\@coadvisorA)} \vspace{1em}\\%
      \fi
      \ifx \@coadvisorBzh \@empty \else
        {\@coadvisorBzh(\@coadvisorB)} \vspace{1em}\\%
      \fi
    \end{tabular}%
    \end{center}
  \vspace{3cm}
  
  \fontsize{18}{27}\Large{\@nation} \Large{\@yearmonth}\\
  \LARGE{\@degreemonth} \ \LARGE{\@degreeyear} \\
  \end{center}
}


\def\titlepage
{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \begin{center}
    \singlespacing\Large
    \@titlezh\\
    \vspace{0.25\baselineskip}
    \@title\\
    \vspace{0.25\baselineskip}
  \end{center}
  \begin{flushleft}
    \singlespacing
    \setlength{\tabcolsep}{0.25em}
    \begin{tabular}{rl}%
      \large{\makebox[4em][s]{研究生}：}&\large{\@authorzh}\vspace{0.1em}\\%
      \large{指導教授：}&{\large{\@advisorzh}}\\%
      \ifx \@coadvisorAzh \@empty \else
        &{\large{\@coadvisorAzh}}\\%
      \fi
      \ifx \@coadvisorBzh \@empty \else
        &{\large{\@coadvisorBzh}}\\%
      \fi
    \end{tabular}%
    \hfill
    \begin{tabular}{ll}%
      \large{Student:}&{\large{\@author}}\vspace{0.5em}\\%
      \large{Advisor:}&{Dr. \large{\@advisor}}\\%
      \ifx \@coadvisorA \@empty \else
        &{\large{\@coadvisorA}}\\%
      \fi
      \ifx \@coadvisorB \@empty \else
        &{\large{\@coadvisorB}}\\%
      \fi
    \end{tabular}
  \end{flushleft}
  \vfill
  \begin{center}
    \large\@universityzh \vspace{-0.5em}\\
    \large\@institutezh \vspace{-0.5em}\\
    \ifTHESISOPTIONdraft
      \large\@thesistypezh \ 初稿\\
    \else
      \large\@thesistypezh\\
    \fi
    \vfill
    \ifTHESISOPTIONdraft
      \centerline{{A Thesis Draft}} \vspace{-1.0em}%
    \else
      \centerline{{A Thesis}} \vspace{-1.0em}%
    \fi
    Submitted to {\@institute} \vspace{-1.0em}\\
    \@college \vspace{-1.0em}\\
    \@university \vspace{-1.0em}\\
    in partial Fulfilment of the Requirements \vspace{-1.0em}\\
    for the Degree of \vspace{-1.0em}\\
    \@degree \vspace{-1.0em}\\
    in \vspace{-1.0em}\\
    \@field \vspace{-1.0em} \\
    \vspace{\baselineskip}
    \vfill
    {{\@degreemonth} {\@degreeyear}}\\
    \@location\\
    \vfill
    \Large{\@nation} \Large{\@yearmonth}
  \end{center}
}


\def\authzpage{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \phantomsection
  \null\newpage
}


\def\approvalzhpage{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \phantomsection
  \null\newpage
}


\def\approvalenpage{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \phantomsection
  \null\newpage
}


\def\copyrightpage{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \rule[0pt]{0pt}{0pt} \\
  \vspace{2.5in}
  \rule[0pt]{0pt}{0pt} \\
  \begin{center}
    \copyright {\@degreeyear} - {\@author}\\
    \vspace{0.5\baselineskip}
    All rights reserved.\\
  \end{center}
}


\def\maketitle{{
\ifTHESISOPTIONreview\else
  \coverpage


  \titlepage
  
  \input{ack/ack}
  

  \frontmatter
  


\fi
}}


\def\abszhpage
{
  \cleardoublepage
  \ifTHESISOPTIONfinal
    \setcounter{page}{\the\numexpr\@reservedfrontpages+\arabic{page}\relax}
  \fi
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{摘要}}
  \begin{center}
    \singlespacing
    {\Large \bf \@titlezh}\\
    \vspace{\baselineskip}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr}%
      \setlength{\tabcolsep}{0.25em}%
      \begin{tabular}{rl}%
        \large{學生：}&{\large{\@authorzh}}\\%
      \end{tabular}&%
      \setlength{\tabcolsep}{0.25em}%
      \begin{tabular}{rlc}%
        \large{指導教授：}&{\large{\@advisorzh}}&{\large{博士}}\\%
        \ifx \@coadvisorAzh \@empty \else
          &{\large{\@coadvisorAzh}}&{\large{博士}}\\%
        \fi
        \ifx \@coadvisorBzh \@empty \else
          &{\large{\@coadvisorBzh}}&{\large{博士}}\\%
        \fi
      \end{tabular}\\%
    \end{tabular*}\\
    \vspace{0.5\baselineskip}
    \large{\@universityzh\hspace{1ex}\@institutezh}\\
    \vspace{\baselineskip}
    \Large{\textbf{摘\qquad 要}}\\
  \end{center}
}

\newenvironment{abstractzh}{%
  \ifTHESISOPTIONreview\else
    \abszhpage
    \par %
  \fi
  \ifTHESISOPTIONreview\comment\fi  %
}{%
  \ifTHESISOPTIONreview\endcomment\fi
}


\def\absenpage
{
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{Abstract}}
  \begin{center}
    \singlespacing
    {\Large \bf \@title}\\
    \vspace{\baselineskip}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr}%
      \setlength{\tabcolsep}{0.25em}%
      \begin{tabular}{rl}%
        \large{Student:}&{\large{\@author}}\\%
      \end{tabular}&%
      \setlength{\tabcolsep}{0.25em}%
      \begin{tabular}{rl}%
        \large{Advisor:}&{\large{Dr. \@advisor}}\\%
        \ifx \@coadvisorA \@empty \else
          &{\large{Dr. \@coadvisorA}}\\%
        \fi
        \ifx \@coadvisorB \@empty \else
          &{\large{Dr. \@coadvisorB}}\\%
        \fi
      \end{tabular}\\%
    \end{tabular*}\\
    \vspace{0.5\baselineskip}
    \large{\@institute}\\
    \large{\@university}\\
    \vspace{\baselineskip}
    \Large{\textbf{Abstract}}\\
  \end{center}
}

\newenvironment{abstract}{%
  \ifTHESISOPTIONreview\else
    \absenpage
    \par %
  \fi
  \ifTHESISOPTIONreview\comment\fi  %
}{%
  \ifTHESISOPTIONreview\endcomment\fi
}


\def\ackpage
{
  \cleardoublepage
  \ClearShipoutPicture  %
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@acktitle}}
  \begin{center}
    \ifTHESISOPTIONzh
      {\LARGE \bf \makebox[3em][s]{\@acktitle}}\\
    \else
      {\LARGE \bf \@acktitle}\\
    \fi
  \end{center}
}

\newenvironment{acknowledgement}{%
  \ifTHESISOPTIONfinal
    \ackpage
    \par %
  \fi
  \ifTHESISOPTIONfinal\else\comment\fi  %
}{%
  \ifTHESISOPTIONfinal\else\endcomment\fi
}


\newenvironment{dedication}{%
  \ifTHESISOPTIONfinal\ifTHESISOPTIONphd
    \cleardoublepage
    \ClearShipoutPicture  %
    \thispagestyle{empty}%
    \vspace*{6.6cm}
    \begin{center}
  \fi\fi
  \ifTHESISOPTIONfinal\ifTHESISOPTIONphd\else\comment\fi\else\comment\fi
}{%
  \ifTHESISOPTIONfinal\ifTHESISOPTIONphd\else\endcomment\fi\else\endcomment\fi
  \ifTHESISOPTIONfinal\ifTHESISOPTIONphd
    \end{center}
  \fi\fi
}


\newenvironment{vita}{%
  \ifTHESISOPTIONreview\comment\else\ifTHESISOPTIONphd\else\comment\fi\fi
    \cleardoublepage
    \phantomsection
    \addcontentsline{toc}{chapter}{\textbf{\@cvtitle}}
    \ifTHESISOPTIONzh
      \chapter*{\makebox[3em][s]{\@cvtitle}}
    \else
      \chapter*{\@cvtitle}
    \fi
}{%
  \ifTHESISOPTIONreview\endcomment\else\ifTHESISOPTIONphd\else\endcomment\fi\fi
}


\newenvironment{publications}{%
  \ifTHESISOPTIONreview\comment\else\ifTHESISOPTIONphd\else\comment\fi\fi
    \cleardoublepage
    \phantomsection
    \addcontentsline{toc}{chapter}{\textbf{\@loptitle}}
    \ifTHESISOPTIONzh
      \chapter*{\makebox[5.5em][s]{\@loptitle}}
    \else
      \chapter*{\@loptitle}
    \fi
}{%
  \ifTHESISOPTIONreview\endcomment\else\ifTHESISOPTIONphd\else\endcomment\fi\fi
}

\endinput

